Adaptive Motion Generation Using Uncertainty-Driven Foresight Prediction

Uncertainty of environments has long been a difficult characteristic to handle, when performing real-world robot tasks. This is because the uncertainty produces unexpected observations that cannot be covered by manual scripting. Learning based robot controlling methods are a promising approach for generating flexible motions against unknown situations, but still tend to suffer under uncertainty due to its deterministic nature. In order to adaptively perform the target task under such conditions, the robot control model must be able to accurately understand the possible uncertainty, and to exploratively derive the optimal action that minimizes such uncertainty. This paper extended an existing predictive learning based robot control method, which employ foresight prediction using dynamic internal simulation. The foresight module refines the model's hidden states by sampling multiple possible futures and replace with the one that led to the lower future uncertainty. The adaptiveness of the model was evaluated on a door opening task. The door can be opened either by pushing, pulling, or sliding, but robot cannot visually distinguish which way, and is required to adapt on the fly. The results showed that the proposed model adaptively diverged its motion through interaction with the door, whereas conventional methods failed to stably diverge. The models were analyzed on Lyapunov exponents of RNN hidden states which reflect the possible divergence at each time step during task execution. The result indicated that the foresight module biased the model to consider future consequences, which lead to embedding uncertainties at the policy of the robot controller, rather than the resultant observation. This is beneficial for implementing adaptive behaviors, which indices derivation of diverse motion during exploration.

==> 00_abstract.tex <==
\begin{abstract}

Uncertainty of environments has long been a difficult characteristic to handle,
when performing real-world robot tasks. This is because the uncertainty produces
unexpected observations that cannot be covered by manual scripting.
Learning based robot controlling methods are a promising approach for generating
flexible motions against unknown situations, but still tend to suffer under uncertainty
due to its deterministic nature. In order to adaptively perform the target
task under such conditions, the robot control model must be able to accurately
understand the possible uncertainty, and to exploratively derive the optimal
action that minimizes such uncertainty. This paper extended a existing predictive
learning based robot control method, which employ foresight prediction using dynamic
internal simulation. The foresight module samples multiple future prediction using 
the dynamics that a Recurrent Neural Network (RNN) has internally structured.
Each foresight starts with a hidden state with random noise applied, so that
multiple possible futures can be explored. The foresights are scored by the predicted
expected variance, or uncertainty, where the one with the lowest value is
selected for actual robot controlling. The adaptiveness of the model was evaluated
on a door opening task. The door can be opened either by pushing, pulling, or sliding,
but robot cannot visually distinguish which way, and is required to adapt on the fly.
The results showed that the proposed model adaptively diverged its motion 
through interaction with the door, whereas conventional methods failed to stably
diverge. The models were analyzed on Lyapunov exponents of RNN hidden states
which reflect the possible divergence at each time step during task execution.
The result indicated that the foresight module biased the model to consider
future consequences, which lead to embedding uncertainties at the policy of
the robot controller, rather than the resultant observation. This is beneficial for
implementing adaptive behaviors, which indices derivation of diverse motion
during exploration.






不確実な環境でロボットが状況を正しく認識し, 行動するには, 探索的な試行錯誤が必要である. 
ただ, 教示データをトレースする模倣学習では, その探索的な性質の獲得が難しい. 本提案では, 
学習モデルが予測する内的不確実性に応じたランダムノイズをモデルの内部状態に加え, 先読みによる
探索的な動作学習を実現する. 実験では提案手法が従来と比べて不確実性に対する適応性が高く, 
効率的な動作学習が可能であることが示された。

\end{abstract}


==> 01_introduction.tex <==

\begin{figure*}[!b]
    \centering
    \includegraphics[width=\linewidth]{assets/fig1.png}
    \caption{Network structure of the proposed model. The model extends the scheme of 
    deep predictive learning by adding a foresight module that alters the hidden states
    of RNNs through closed-loop predictions. }
    \label{fig:model_structure}
\end{figure*}

\section{INTRODUCTION}

In the field of robot controlling, introduction of deep learning methods has enlarged the
application area of robot task execution. One representative approach is learning from
demonstration (LfD), where neural network models are trained to capture the dynamics of target
tasks through imitation of given demonstration data \cite{itosan}. LfD benefits from its
training-efficiency, as robust and flexible robot motions can be acquired from a few set of
demonstrations.

However, task environments may embrace hidden properties that cannot be fully covered
by the demonstrations. One example is a door opening task, where the robot is trained to
open the door without knowing which direction the door could be opened (i.e., pushing
or pulling). As it is difficult for LfD methods to incorporate failure demonstrations,
such as pushing a pull door by mistake, the method's generalization ability becomes limited
under such uncertain environments.


In order to enable generalization under uncertainty, \textit{adaptiveness} of the robot
control model becomes important. This is because the uncertainty can be reduced through
online-adaptation to the environment, which requires to actively interact and change the policy
based on the feedback. Therefore, the robot control models must be equipped with motivations to
(1) correctly understand the dynamic uncertainty of the environment and to (2) exploratively
derive the optimal action. 

Previous research \cite{srnn} proposed a model structure that jointly captures the temporal
dynamics of the task and its time-dependent uncertainty. But the deterministic nature of
Recurrent Neural Networks (RNN) limited the derivation of explorative behaviors. Other
researches introduced Active Inference for exploration, which samples and select actions based
on scores that reflect extrinsic reward and intrinsic information gain \cite{ai1}. However,
the methods required pre-defined uncertainty models and small actions space, hence suffer
in dynamic real-robot applications. Although recent researches \cite{diffusion_policy, pv_rnn}
enabled both properties (i.e., capturing the dynamic uncertainties and implementing explorative
behaviors) in real-robot tasks, their slow inference speed limits the application targets.

This paper proposes a deep predictive learning \cite{predictive_learning} based motion generation
model that applies adaptiveness for learning tasks with uncertainty. The proposed model extends
the conventional RNN models to enable exploration by predicting multiple foresights, where the
one that had the lowest expected uncertainty, or variance, will be selected for action generation.
As the predicted foresights vary depending on the current predicted uncertainty, the trained model
will acquire adaptiveness, predicting explorative foresights when the uncertainty is higher.



==> 05_conclusion.tex <==
\section{CONCLUSION}

This paper introduced a foresight prediction module to an RNN-based predictive 
learning model. The experiment results suggested that this module enabled stable
prediction under uncertain environment, by biasing the model to embed uncertainty
in policy selection, which induced active and explorative motion generation.

